Phonon Assisted Exciton Processes in Two-Dimensional Tungsten Monocarbide

n this study, we utilize a rigorous ab initio-based finite momentum Bethe-Salpeter equation to investigate the photoluminescence emission in two-dimensional hexagonal tungsten carbide (h-WC). This thermodynamically stable monolayer exhibits an indirect optical gap, resulting in phonon-assisted emission. We observe that light absorption is a direct process centered around the direct quasiparticle gap, while light emission is indirect and requires modes between $\Gamma$-$M$ in the phonon dispersion. The emission lines feature prominent phonon replicas at cryogenic temperatures, particularly near-infrared wavelengths (1.09 and 1.17 eV), and we observe exciton thermalization with the crystal beyond 25 K. Additionally, non-radiative recombination is a remarkably fast process, occurring at order of a few femtoseconds (4.8 fs at 0 K and 2.8 fs at 300 K) compared to radiative recombination (2.3 ps at 0 K and 214 ns at 300 K). These optical characteristics of 2D h-WC may facilitate the promise of photon-emitter devices for near-infrared signal communication.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
